Necessary and Sufficient Girth Conditions for LDPC Tanner Graphs with Denser Protographs

This paper gives necessary and sufficient conditions for the Tanner graph of a quasi-cyclic (QC) low-density parity-check (LDPC) code based on the all-one protograph to have girth 6, 8, 10, and 12, respectively, in the case of parity-check matrices with column weight 4. These results are a natural extension of the girth results of the already-studied cases of column weight 2 and 3, and it is based on the connection between the girth of a Tanner graph given by a parity-check matrix and the properties of powers of the product between the matrix and its transpose. The girth conditions can be easily incorporated into fast algorithms that construct codes of desired girth between 6 and 12; our own algorithms are presented for each girth, together with constructions obtained from them and corresponding computer simulations. More importantly, this paper emphasizes how the girth conditions of the Tanner graph corresponding to a parity-check matrix composed of circulants relate to the matrix obtained by adding (over the integers) the circulant columns of the parity-check matrix. In particular, we show that imposing girth conditions on a parity-check matrix is equivalent to imposing conditions on a square circulant submatrix of size 4 obtained from it.

==> backupstufffromend.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%
%% Some comments about useful packages
%% (extract from bare_conf.tex by Michael Shell)
%%

% *** MISC UTILITY PACKAGES ***
%
%\usepackage{ifpdf}
% Heiko Oberdiek's ifpdf.sty is very useful if you need conditional
% compilation based on whether the output is pdf or dvi.
% usage:
% \ifpdf
%   % pdf code
% \else
%   % dvi code
% \fi
% The latest version of ifpdf.sty can be obtained from:
% http://www.ctan.org/pkg/ifpdf
% Also, note that IEEEtran.cls V1.7 and later provides a builtin
% \ifCLASSINFOpdf conditional that works the same way.
% When switching from latex to pdflatex and vice-versa, the compiler may
% have to be run twice to clear warning/error messages.


% *** CITATION PACKAGES ***
%
%\usepackage{cite}
% cite.sty was written by Donald Arseneau
% V1.6 and later of IEEEtran pre-defines the format of the cite.sty package
% \cite{} output to follow that of the IEEE. Loading the cite package will
% result in citation numbers being automatically sorted and properly
% "compressed/ranged". e.g., [1], [9], [2], [7], [5], [6] without using
% cite.sty will become [1], [2], [5]--[7], [9] using cite.sty. cite.sty's
% \cite will automatically add leading space, if needed. Use cite.sty's
% noadjust option (cite.sty V3.8 and later) if you want to turn this off
% such as if a citation ever needs to be enclosed in parenthesis.
% cite.sty is already installed on most LaTeX systems. Be sure and use
% version 5.0 (2009-03-20) and later if using hyperref.sty.
% The latest version can be obtained at:
% http://www.ctan.org/pkg/cite
% The documentation is contained in the cite.sty file itself.


% *** GRAPHICS RELATED PACKAGES ***
%
\ifCLASSINFOpdf
  % \usepackage[pdftex]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../pdf/}{../jpeg/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.pdf,.jpeg,.png}
\else
  % or other class option (dvipsone, dvipdf, if not using dvips). graphicx
  % will default to the driver specified in the system graphics.cfg if no
  % driver is specified.
  % \usepackage[dvips]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../eps/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.eps}
\fi
% graphicx was written by David Carlisle and Sebastian Rahtz. It is
% required if you want graphics, photos, etc. graphicx.sty is already
% installed on most LaTeX systems. The latest version and documentation
% can be obtained at: 
% http://www.ctan.org/pkg/graphicx
% Another good source of documentation is "Using Imported Graphics in
% LaTeX2e" by Keith Reckdahl which can be found at:
% http://www.ctan.org/pkg/epslatex
%
% latex, and pdflatex in dvi mode, support graphics in encapsulated
% postscript (.eps) format. pdflatex in pdf mode supports graphics
% in .pdf, .jpeg, .png and .mps (metapost) formats. Users should ensure
% that all non-photo figures use a vector format (.eps, .pdf, .mps) and
% not a bitmapped formats (.jpeg, .png). The IEEE frowns on bitmapped formats
% which can result in "jaggedy"/blurry rendering of lines and letters as
% well as large increases in file sizes.
%
% You can find documentation about the pdfTeX application at:
% http://www.tug.org/applications/pdftex


% *** MATH PACKAGES ***
%
%\usepackage{amsmath}
% A popular package from the American Mathematical Society that provides
% many useful and powerful commands for dealing with mathematics.
%
% Note that the amsmath package sets \interdisplaylinepenalty to 10000
% thus preventing page breaks from occurring within multiline equations. Use:
%\interdisplaylinepenalty=2500
% after loading amsmath to restore such page breaks as IEEEtran.cls normally
% does. amsmath.sty is already installed on most LaTeX systems. The latest
% version and documentation can be obtained at:
% http://www.ctan.org/pkg/amsmath


% *** SPECIALIZED LIST PACKAGES ***
%
%\usepackage{algorithmic}
% algorithmic.sty was written by Peter Williams and Rogerio Brito.
% This package provides an algorithmic environment fo describing algorithms.
% You can use the algorithmic environment in-text or within a figure
% environment to provide for a floating algorithm. Do NOT use the algorithm
% floating environment provided by algorithm.sty (by the same authors) or
% algorithm2e.sty (by Christophe Fiorio) as the IEEE does not use dedicated
% algorithm float types and packages that provide these will not provide
% correct IEEE style captions. The latest version and documentation of
% algorithmic.sty can be obtained at:
% http://www.ctan.org/pkg/algorithms
% Also of interest may be the (relatively newer and more customizable)
% algorithmicx.sty package by Szasz Janos:
% http://www.ctan.org/pkg/algorithmicx


% *** ALIGNMENT PACKAGES ***
%
%\usepackage{array}
% Frank Mittelbach's and David Carlisle's array.sty patches and improves
% the standard LaTeX2e array and tabular environments to provide better
% appearance and additional user controls. As the default LaTeX2e table
% generation code is lacking to the point of almost being broken with
% respect to the quality of the end results, all users are strongly
% advised to use an enhanced (at the very least that provided by array.sty)
% set of table tools. array.sty is already installed on most systems. The
% latest version and documentation can be obtained at:
% http://www.ctan.org/pkg/array

% IEEEtran contains the IEEEeqnarray family of commands that can be used to
% generate multiline equations as well as matrices, tables, etc., of high
% quality.


% *** SUBFIGURE PACKAGES ***
%\ifCLASSOPTIONcompsoc
%  \usepackage[caption=false,font=normalsize,labelfont=sf,textfont=sf]{subfig}
%\else
%  \usepackage[caption=false,font=footnotesize]{subfig}
%\fi
% subfig.sty, written by Steven Douglas Cochran, is the modern replacement
% for subfigure.sty, the latter of which is no longer maintained and is
% incompatible with some LaTeX packages including fixltx2e. However,
% subfig.sty requires and automatically loads Axel Sommerfeldt's caption.sty
% which will override IEEEtran.cls' handling of captions and this will result
% in non-IEEE style figure/table captions. To prevent this problem, be sure
% and invoke subfig.sty's "caption=false" package option (available since
% subfig.sty version 1.3, 2005/06/28) as this is will preserve IEEEtran.cls
% handling of captions.
% Note that the Computer Society format requires a larger sans serif font
% than the serif footnote size font used in traditional IEEE formatting
% and thus the need to invoke different subfig.sty package options depending
% on whether compsoc mode has been enabled.
%
% The latest version and documentation of subfig.sty can be obtained at:
% http://www.ctan.org/pkg/subfig


% *** FLOAT PACKAGES ***
%
%\usepackage{fixltx2e}
% fixltx2e, the successor to the earlier fix2col.sty, was written by
% Frank Mittelbach and David Carlisle. This package corrects a few problems
% in the LaTeX2e kernel, the most notable of which is that in current
% LaTeX2e releases, the ordering of single and double column floats is not
% guaranteed to be preserved. Thus, an unpatched LaTeX2e can allow a
% single column figure to be placed prior to an earlier double column
% figure.
% Be aware that LaTeX2e kernels dated 2015 and later have fixltx2e.sty's
% corrections already built into the system in which case a warning will
% be issued if an attempt is made to load fixltx2e.sty as it is no longer
% needed.
% The latest version and documentation can be found at:
% http://www.ctan.org/pkg/fixltx2e


%\usepackage{stfloats}
% stfloats.sty was written by Sigitas Tolusis. This package gives LaTeX2e
% the ability to do double column floats at the bottom of the page as well
% as the top. (e.g., "\begin{figure*}[!b]" is not normally possible in
% LaTeX2e). It also provides a command:
%\fnbelowfloat
% to enable the placement of footnotes below bottom floats (the standard
% LaTeX2e kernel puts them above bottom floats). This is an invasive package
% which rewrites many portions of the LaTeX2e float routines. It may not work
% with other packages that modify the LaTeX2e float routines. The latest
% version and documentation can be obtained at:
% http://www.ctan.org/pkg/stfloats
% Do not use the stfloats baselinefloat ability as the IEEE does not allow
% \baselineskip to stretch. Authors submitting work to the IEEE should note
% that the IEEE rarely uses double column equations and that authors should try
% to avoid such use. Do not be tempted to use the cuted.sty or midfloat.sty
% packages (also by Sigitas Tolusis) as the IEEE does not format its papers in
% such ways.
% Do not attempt to use stfloats with fixltx2e as they are incompatible.
% Instead, use Morten Hogholm'a dblfloatfix which combines the features
% of both fixltx2e and stfloats:
%
% \usepackage{dblfloatfix}
% The latest version can be found at:
% http://www.ctan.org/pkg/dblfloatfix


% *** PDF and URL PACKAGES ***
%
%\usepackage{url}
% url.sty was written by Donald Arseneau. It provides better support for
% handling and breaking URLs. url.sty is already installed on most LaTeX
% systems. The latest version and documentation can be obtained at:
% http://www.ctan.org/pkg/url
% Basically, \url{my_url_here}.



% *** Do not adjust lengths that control margins, column widths, etc. ***
% *** Do not use packages that alter fonts (such as pslatex).         ***
%%%%%%


%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


\begin{remark} Note that the transpose of the matrix $$\begin{bmatrix} n_vI & C_{12} &C_{13}&C_{14} \end{bmatrix} $$ is equal to the sum of the $n_v$ circulant columns of $H$. 
\end{remark}

\begin{theorem}
\label{girthH>4}
Let $H(x)$ and $C_H(x)$ be defined as in equations \eqref{polynomialpcheckmatrix} and \eqref{polynomialC_H}, respectively. Then $\mathrm{girth}(H(x))>4$ if and only if each one of the six sets $\{0,i_2,i_3,\dots,i_{n_v}\}$, $\{0,j_2,j_3,\dots,j_{n_v}\}$, $\{0,k_2,k_3,\dots,k_{n_v}\}$, $\{0,i_2-j_2,i_3-j_3,\dots,i_{n_v}-j_{n_v}\}$, $\{0,i_2-k_2,i_3-k_3,\dots,i_{n_v}-k_{n_v}\}$ and $\{0,j_2-k_2,j_3-k_3,\dots,j_{n_v}-k_{n_v}\}$ contains exactly $n_v$ distinct elements.
\end{theorem}

\proof By Theorem \ref{theorem_girth}, $\text{girth}(H)>4$ if and only if $C_H\triangle0=0$. This is equivalent to have $C_{ij}(x)\triangle0=0$ for all $1\leq i<j\leq4$. If we expand each of these equations, we obtain
%{\centering
%\begin{multicols}{2}
$$ \sum_{l=1}^{n_v}x^{i_l}\triangle0=0, \quad \sum_{l=1}^{n_v}x^{j_l}\triangle 0=0,\quad 
 \sum_{l=1}^{n_v}x^{k_l}\triangle0=0$$ 
$$ \sum_{l=1}^{n_v}x^{i_l-j_l} \triangle0=0, \quad \sum_{l=1}^{n_v}x^{i_l-k_l} \triangle 0=0, \quad 
\sum_{l=1}^{n_v}x^{j_l-k_l}\triangle0=0$$
%\end{multicols}
%}

\noindent By using the definition of the triangle operator $\triangle$, we conclude that, for each equation, the exponents should be distinct and the claim follows. \qed

\

\noindent To choose the exponents $i_l, j_l$ and $k_l$ satisfying the conditions in Theorem \ref{girthH>4}, we provide the following recursive algorithm. In this algorithm, we choose first $i_1,j_1,k_1$, then we choose $i_2,j_2,k_2$, then we choose $i_3,j_3,k_3$, and so on.

\begin{Algorithm}
\label{algorithmgirth4}
%To construct the polynomial parity-check matrix $H(x)$ with $\text{girth}(H(x))>4$, consider the following steps.

\

\noindent Step 1: Set $i_1=0$, $j_1=0$ and $k_1=0$. Set $l=1$.

\noindent Step 2: Let $l:=l+1$. Choose

%\noindent $i_l\notin \{i_1,i_2,\dots,i_{l-1}\}$
\noindent $i_l\notin \{i_m \mid 1\leq m\leq l-1\}$

%\noindent $j_l\notin \{j_1,j_2,\dots,j_{l-1}\} \cup \{i_l+(j_1-i_1),i_l+(j_2-i_2),\dots,i_l+(j_{l-1}-i_{l-1})\}$
\noindent $j_l\notin \{j_m \mid 1\leq m\leq l-1\} \cup \{i_l+(j_m-i_m) \mid 1\leq m\leq l-1\}$

%\noindent $k_l\notin \{k_1,k_2,\dots,k_{l-1}\} \cup \{i_l+(k_1-i_1),i_l+(k_2-i_2),\dots,i_l+(k_{l-1}-i_{l-1})\} \cup \{j_l+(k_1-j_1),j_l+(k_2-j_2),\dots,j_l+(k_{l-1}-j_{l-1})\}$
\noindent $k_l\notin \{k_m \mid 1\leq m\leq l-1\} \cup \{i_l+(k_m-i_m) \mid 1\leq m\leq l-1\} \cup \{j_l+(k_m-j_m) \mid 1\leq m\leq l-1\}$

\noindent Step 3: If $l=n_v$ stop; otherwise go to Step 2.
\end{Algorithm}

%\

\begin{example}
\label{example1_girth4}
In this example, we construct a $4\times6$ protograph-based matrix using Algorithm \ref{algorithmgirth4}. In each iteration $l$, $2\leq l\leq n_v$, we choose the smallest positive value for each of $i_l,j_l$ and $k_l$. We obtain 
$$H(x)=\left(\begin{matrix} 1&1&1&1&1&1 \\ 1&x&x^2&x^3&x^4&x^5 \\ 1&x^2&x&x^5&x^7&x^3 \\ 1&x^3&x^5&x&x^9&x^2 \end{matrix}\right).$$
\noindent If we choose lifting degree $N=\displaystyle \left(\max_{1\leq l\leq6}\{i_l,j_l,k_l\}\right)+1=10$, then $H(x)$ has girth 6. %\qed
\end{example}

%\

\begin{example}
\label{example2_girth4}
Using Algorithm \ref{algorithmgirth4}, we construct a protograph-based matrix as in Example \ref{example1_girth4}. In each iteration $l$, $2\leq l\leq n_v$, however, we choose each of $i_l,j_l$ and $k_l$ to be one more than the maximum value in their corresponding forbidden sets. We obtain  
$$H(x)=\left(\begin{matrix} 1&1&1&1&1&1 \\ 1&x&x^2&x^3&x^4&x^5 \\ 1&x^2&x^4&x^6&x^8&x^{10} \\ 1&x^3&x^6&x^9&x^{12}&x^{15} \end{matrix}\right).$$
\noindent If we let $N=\displaystyle \left(\max_{1\leq l\leq6}\{i_l,j_l,k_l\}\right)+1=16$, then the girth of $H(x)$ is 6. Notice that $N=16$ is not the smallest positive value for which $\text{girth}(H(x))>4$. If we choose $N=7$, then $\text{girth}(H(x))=6$. %\qed
\end{example}

%\

\begin{theorem}
\label{girthH>6}
Let $H(x)$ and $C_H(x)$ be defined as in equations \eqref{polynomialpcheckmatrix} and \eqref{polynomialC_H}, respectively. Then $\mathrm{girth}(H(x))>6$ if and only if $\mathrm{girth}(H(x))>4$ and, for any $m\in[n_v]$, each one of the four sets

\

\textbf{\textcolor{red}{REWRITE THESE SETS IN A BETTER WAY TO REDUCE SPACE}}

$\{i_m-i_n \mid n\in[n_v], n\neq m\} \cup \{j_m-j_p \mid p\in[n_v], p\neq m\} \cup \{k_m-k_q \mid q\in[n_v], q\neq m\}$

\

$\{i_n \mid n\in[n_v], n\neq m\} \cup \{i_p-j_p+j_m \mid p\in[n_v], p\neq m\} \cup \{i_q-k_q+k_m \mid q\in[n_v], q\neq m\} \cup \{i_p+(j_n-j_m)+(k_m-k_p) \mid n,p\in[n_v], p\neq m,n\neq m\}$
%\begin{multline}
%\{i_n \mid n\in[n_v], n\neq m\} \cup \{i_p-j_p+j_m \mid p\in[n_v], p\neq m\} \cup \{i_q-k_q+k_m \mid q\in[n_v], q\neq m\} \\ \cup \{i_p+(j_n-j_m)+(k_m-k_p) \mid n,p\in[n_v], p\neq m,n\neq m\}
%\end{multline}

\

$\{j_n \mid n\in[n_v], n\neq m\} \cup \{j_p-i_p+i_m \mid p\in[n_v], p\neq m\} \cup \{j_q-k_q+k_m \mid q\in[n_v], q\neq m\} \cup \{j_p+(i_n-i_m)+(k_m-k_p) \mid n,p\in[n_v], p\neq m,n\neq m\}$

\

$\{k_n \mid n\in[n_v], n\neq m\} \cup \{k_p-i_p+i_m \mid p\in[n_v], p\neq m\} \cup \{k_q-j_q+j_m \mid q\in[n_v], q\neq m\} \cup \{k_p+(i_n-i_m)+(j_m-j_p) \mid n,p\in[n_v], p\neq m,n\neq m\}$

\

\noindent contains distinct elements.
\end{theorem}

\begin{Algorithm}
\label{algorithmgirth6}
%The conditions to obtain girth(H)>4 are satisfied by these conditions. You can double check with the algorithm.

\

%{\centering \textbf{Check if the conditions for girth$>$4 are satisfied. I double-checked, but just to make sure. Also check if it is required to divide the conditions with indices between 1 and $l-1$, and between $1$ and $l$. See algorithm for $\text{girth}>8.$} \\}
%
%\
%
\noindent Step 1: Set $i_1=0$, $j_1=0$ and $k_1=0$. Set $l=1$.

\noindent Step 2: Let $l:=l+1$. Choose

\noindent $i_l\notin \{i_m, (i_m-j_m)+j_n, (j_m-k_m)+(k_n-j_n)+i_p, (i_m-k_m)+k_n, (k_m-j_m)+(j_n-k_n)+i_p \mid 1\leq m,n,p\leq l-1\}$

\noindent $j_l\notin \{j_m, i_l+j_m-i_n, i_m+(j_n-i_n), (i_m-k_m)+(k_n-i_n)+j_p, i_l+(k_m-i_m)+(j_n-k_n), (j_m-k_m)+k_n, i_l+(j_m-k_m)+k_n-i_p, 2i_l+(k_m-i_m)+(j_n-k_n)-i_p \mid 1\leq m,n,p\leq l-1\}$

\noindent $k_l\notin \{k_m, j_l+k_m-j_n, i_l+k_m-i_n, j_l+(i_m-j_m)+(i_n-k_n), i_m+(k_n-i_n), j_l+i_m-j_n+(k_p-i_p), 2j_l+(i_m-j_m)+(k_n-i_n)-j_p, (k_m-j_m)+j_n, i_l+(j_m-i_m)+(k_n-j_n), i_l+(k_m-j_m)+j_n-i_p, 2i_l+(j_m-i_m)+(k_n-j_n)-i_p \mid 1\leq m,n,p\leq l-1\}$

\noindent Step 3: If $l=n_v$ stop; otherwise go to Step 2.
\end{Algorithm}

%\

\begin{example}
\label{example1_girth6}
In this example, we construct a $4\times6$ protograph-based matrix using Algorithm \ref{algorithmgirth6}. In each iteration $l$, $2\leq l\leq n_v$, we choose the smallest positive value for each of $i_l,j_l$ and $k_l$ as we did in Example \ref{example1_girth4}. Let 

\

{\centering $H(x)=\left(\begin{matrix} 1&1&1&1&1&1 \\ 1&x&x^5&x^8&x^{10}&x^{25} \\ 1&x^3&x^{14}&x^{29}&x^{49}&x^{96} \\ 1&x^4&x^2&x^{36}&x^{55}&x^{108} \end{matrix}\right).$ \\}

\

\noindent If we choose lifting degree $N=\displaystyle \left(\max_{1\leq l\leq6}\{i_l,j_l,k_l\}\right)+1=109$, then $H(x)$ has girth 8. The smallest positive integer $N$ required to obtain $\text{girth}(H(x))>6$ is $N=85$. %\qed
\end{example}

%\

\begin{example}
\label{example2_girth6}
If instead of choosing the smallest positive value for each of $i_l,j_l$ and $k_l$, as in Example \ref{example1_girth6}, we choose one more than the maximum value in their corresponding forbidden sets, we obtain the following matrix

\

{\centering $H(x)=\left(\begin{matrix} 1&1&1&1&1&1 \\ 1&x&x^8&x^{54}&x^{355}&x^{2324} \\ 1&x^3&x^{23}&x^{154}&x^{1011}&x^{6617} \\ 1&x^7&x^{53}&x^{354}&x^{2323}&x^{15203} \end{matrix}\right).$ \\} %\overset{\text{mod} \; 111}{\longrightarrow} \left(\begin{matrix} 1&1&1&1&1&1 \\ 1&x&x^8&x^{54}&x^{22}&x^{104} \\ 1&x^3&x^{23}&x^{43}&x^{12}&x^{68} \\ 1&x^7&x^{53}&x^{21}&x^{103}&x^{107} \end{matrix}\right).$ \\}

\

\noindent If we choose the lifting degree $N=111$, then the matrix $H(x)$ has girth $8$. In fact, this is the smallest value required to obtain this girth. % The next two values required to produce girth = 8 is N=171 and 198.
%The matrix on the right is obtained from $H(x)$ by taking the exponents modulo 111 and it has girth 8 for $N=111$.
If we reduce the exponents modulo 111, we obtain the matrix

\

{\centering $H(x)=\left(\begin{matrix} 1&1&1&1&1&1 \\ 1&x&x^8&x^{54}&x^{22}&x^{104} \\ 1&x^3&x^{23}&x^{43}&x^{12}&x^{68} \\ 1&x^7&x^{53}&x^{21}&x^{103}&x^{107} \end{matrix}\right).$ \\}

\

\noindent In this case we also have $\text{girth}(H(x))=8$ for $N=111$.
\end{example}

%\

\begin{theorem}
\label{girthH>8}
Let $H(x)$ and $C_H(x)$ be defined as in equations \eqref{polynomialpcheckmatrix} and \eqref{polynomialC_H}, respectively. Then $\mathrm{girth}(H(x))>8$ if and only if $\mathrm{girth}(H(x))>4$ and each one of the following sixteen sets

\

\textbf{\textcolor{red}{REWRITE THESE SETS IN A BETTER WAY TO REDUCE SPACE}}

$\{i_u-i_w,j_u-j_w,k_u-k_w \mid u,w\in[n_v], u\neq w\}$

\

$\{i_u-i_w,(i_u-j_u)-(i_w-j_w),(i_u-k_u)-(i_w-k_w) \mid u,w\in[n_v], u\neq w\}$

\

$\{j_u-j_w,(i_u-j_u)-(i_w-j_w),(j_u-k_u)-(j_w-k_w) \mid u,w\in[n_v], u\neq w\}$

\

$\{k_u-k_w,(i_u-k_u)-(i_w-k_w),(j_u-k_u)-(j_w-k_w) \mid u,w\in[n_v], u\neq w\}$

\

$\{(i_u-j_u)+j_w,(i_u-k_u)+k_w \mid u,w\in[n_v], u\neq w\}$

\

$\{(j_u-i_u)+i_w,(j_u-k_u)+k_w \mid u,w\in[n_v], u\neq w\}$

\

$\{(k_u-i_u)+i_w,(k_u-j_u)+j_w \mid u,w\in[n_v], u\neq w\}$

\

$\{(j_u-i_u)-j_w,(k_u-i_u)-k_w \mid u,w\in[n_v], u\neq w\}$

\

$\{j_u-i_w,(j_u-k_u)-(i_w-k_w) \mid u,w\in[n_v], u\neq w\}$

\

$\{k_u-i_w,(k_u-j_u)-(i_w-j_w) \mid u,w\in[n_v], u\neq w\}$

\

$\{(i_u-j_u)-i_w,(k_u-j_u)-k_w \mid u,w\in[n_v], u\neq w\}$

\

$\{i_u-j_w,(i_u-k_u)-(j_w-k_w) \mid u,w\in[n_v], u\neq w\}$

\

$\{k_u-j_w,(k_u-i_u)-(j_w-i_w) \mid u,w\in[n_v], u\neq w\}$

\

$\{(i_u-k_u)-i_w,(j_u-k_u)-j_w \mid u,w\in[n_v], u\neq w\}$

\

$\{i_u-k_w,(i_u-j_u)-(k_w-j_w) \mid u,w\in[n_v], u\neq w\}$

\

$\{j_u-k_w,(j_u-i_u)-(k_w-i_w) \mid u,w\in[n_v], u\neq w\}$

\

\noindent contains distinct elements. %\textbf{THIS IS INCOMPLETE. THE NON-DIAGONAL CONDITIONS ALSO CONTRIBUTE.}
\end{theorem}

%\

\begin{example}
\label{example1_girth8}
In this example, we construct a $4\times6$ protograph-based matrix using an algorithm derived from Theorem \ref{girthH>8}. In each iteration $l$, $2\leq l\leq n_v$, we choose the smallest positive value for each of $i_l,j_l$ and $k_l$ as we did in Examples \ref{example1_girth4} and \ref{example1_girth6}. Let 

\

{\centering $H(x)=\left(\begin{matrix} 1&1&1&1&1&1 \\ 1&x&x^9&x^{28}&x^{41}&x^{75} \\ 1&x^3&x^{21}&x^{54}&x^{98}&x^{180} \\ 1&x^7&x^{38}&x^{93}&x^{162}&x^{297} \end{matrix}\right).$ \\}

\

\noindent If we choose $N=\displaystyle 2\left(\max_{1\leq l\leq6}\{i_l,j_l,k_l\}\right)+1=595$, then $H(x)$ has girth 10. The smallest positive integer $N$ required to obtain $\text{girth}(H(x))>8$ is $N=347$. %\qed
\end{example}

%\

\begin{theorem}
\label{girthH>10}
Let $H(x)$ and $C_H(x)$ be defined as in equations \eqref{polynomialpcheckmatrix} and \eqref{polynomialC_H}, respectively. Then $\mathrm{girth}(H(x))>10$ if and only if $\mathrm{girth}(H(x))>8$ and, for any $l\in[n_v]$, each one of the four sets

\

$\{i_u-i_w, j_u-j_w, k_u-k_w, i_l+(j_u-i_u)-j_w, i_l+(k_u-i_u)-k_w, j_l+(i_u-j_u)-i_w, j_l+(k_u-j_u)-k_w, k_l+(i_u-k_u)-i_w, k_l+(j_u-k_u)-j_w \mid u,w\in[n_v], u\neq w, u\neq l\}$

\

$\{(i_u-j_u)+j_w, (i_u-k_u)+k_w, i_l+i_u-i_w, i_l+(i_u-j_u)-(i_w-j_w), i_l+(i_u-k_u)-(i_w-k_w), j_l+i_u-j_w, j_l+(i_u-k_u)-(j_w-k_w), k_l+i_u-k_w, k_l+(i_u-j_u)-(k_w-j_w) \mid u,w\in[n_v], u\neq w, w\neq l\}$

\

$\{(j_u-i_u)+i_w, (j_u-k_u)+k_w, i_l+j_u-i_w, i_l+(j_u-k_u)-(i_w-k_w), j_l+j_u-j_w, j_l+(i_w-j_w)-(i_u-j_u), j_l+(j_u-k_u)-(j_w-k_w), k_l+j_u-k_w, k_l+(j_u-i_u)-(k_w-i_w) \mid u,w\in[n_v], u\neq w, w\neq l\}$

\

$\{(k_u-i_u)+i_w, (k_u-j_u)+j_w, i_l+k_u-i_w, i_l+(k_u-j_u)-(i_w-j_w), j_l+k_u-j_w, j_l+(k_u-i_u)-(j_w-i_w), k_l+k_u-k_w, k_l+(i_w-k_w)-(i_u-k_u), k_l+(j_w-k_w)-(j_u-k_u) \mid u,w\in[n_v], u\neq w, w\neq l\}$

\

\noindent contains distinct elements.
\end{theorem}

%\

\begin{example}
\label{example1_girth10}
In this example, we construct a $4\times6$ protograph-based matrix using an algorithm derived from Theorem \ref{girthH>10}. In each iteration $l$, $2\leq l\leq n_v$, we choose the smallest positive value for each of $i_l,j_l$ and $k_l$. Let 

\

{\centering $H(x)=\left(\begin{matrix} 1&1&1&1&1&1 \\ 1&x&x^{12}&x^{45}&x^{147}&x^{445} \\ 1&x^3&x^{31}&x^{126}&x^{320}&x^{980} \\ 1&x^7&x^{67}&x^{231}&x^{636}&x^{1626} \end{matrix}\right).$ \\}

\

\noindent If we choose lifting degree $N=\displaystyle 2\left(\max_{1\leq l\leq6}\{i_l,j_l,k_l\}\right)+1=3253$, then $H(x)$ has girth 12. The smallest positive integer $N$ required to obtain $\text{girth}(H(x))>10$ is $N=1881$.
\end{example}

\bibliographystyle{IEEEtran}
\bibliography{newprefs.bib}%, ../Bib-Files/huge.bib}

\end{document}


